Skip the Compressor: Coding Agents Fix More Issues When They Pick Whole Files

A coding agent works on repositories that can be far larger than its context window can hold. Prompt compressors and retrievers offer solutions to this problem, but patching an issue needs two things at once: the files that must change, and their code exactly as written, since the model must reproduce the lines it edits. Retrievers rank code by its similarity to the issue rather than by whether it must change, and compressors delete text to fit the budget. We show that at an equal token budget, an agent resolves more issues when the budget goes to choosing which files to show verbatim, as our simple selector CQ2-CARE does, than when it goes to pruning tokens or retrieving chunks. We fit every context to the same per-issue budget on 300 recent SWE-rebench issues and grade each patch with the benchmark's tests. With GPT-5.6 and Claude Opus 5, CQ2-CARE resolves 43.7% and 46.7% of the issues, 6.3 points more than the best of three compressors with either model, and 9.3 and 12.7 points more than the best of three retrievers. CQ2-CARE even resolves more issues than two methods trained for issue resolution, SweRank (by 0.7 and 1.7 points) and SWE-Pruner (by 2.0 and 7.3). Our analysis shows the defects of the baseline methods: retrievers often miss the files to edit, and compressors keep them but alter their text, so fewer patches apply. Exact-file selection needs no compression model and shows every line as the repository has it, so the model can quote the code it edits.

==> generated/table_arms.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{1.6pt}
\begin{tabular}{lrrrrrrrrr}
\toprule
Context & Resolved [95\% CI] & Parse & Applies & Res.$|$app. & Mean tok. & Med.\ tok. & In $\pm$2\% & \$/issue & Build s \\
\midrule
Ours (CQ2-CARE) & 43.7 [38.2, 49.3] & 100.0 & 98.0 & 44.6 & 13,778 & 9,377 & not fitted & 0.151 & 0 \\
Single draw (Q50-CARE) & 46.3 [40.8, 52.0] & 100.0 & 98.0 & 47.3 & 20,143 & 15,168 & not fitted & 0.199 & 0 \\
Single draw, size-matched & 42.7 [37.2, 48.3] & 100.0 & 98.0 & 43.5 & 13,262 & 9,275 & not fitted & 0.121 & 0 \\
Ours without evidence & 40.7 [35.3, 46.3] & 100.0 & 97.7 & 41.6 & 10,367 & 5,756 & not fitted & 0.103 & 0 \\
Union of two draws & 47.7 [42.1, 53.3] & 100.0 & 97.7 & 48.8 & 16,123 & 10,705 & not fitted & 0.153 & 0 \\
LLMLingua-2 & 30.0 [25.1, 35.4] & 99.7 & 70.7 & 42.5 & 13,070 & 8,730 & 73.7 & 0.177 & 13 CPU \\
LongLLMLingua & 35.0 [29.8, 40.6] & 100.0 & 84.0 & 41.7 & 13,154 & 8,788 & 66.0 & 0.176 & 37 GPU \\
LongCodeZip & 37.3 [32.1, 42.9] & 99.3 & 89.7 & 41.6 & 13,126 & 8,930 & 65.7 & 0.168 & 34 GPU \\
BM25 (chunks) & 29.0 [24.2, 34.4] & 100.0 & 86.7 & 33.5 & 13,610 & 9,350 & 98.0 & 0.099 & 0 \\
Dense (chunks) & 22.7 [18.3, 27.7] & 99.7 & 78.3 & 28.9 & 13,659 & 9,354 & 99.0 & 0.106 & 15 GPU \\
{\color{gray}\textit{Gold files (upper bound)}} & {\color{gray}\textit{49.3 [43.7, 55.0]}} & {\color{gray}\textit{100.0}} & {\color{gray}\textit{97.7}} & {\color{gray}\textit{50.5}} & {\color{gray}\textit{12,206}} & {\color{gray}\textit{6,556}} & {\color{gray}\textit{not fitted}} & {\color{gray}\textit{0.075}} & {\color{gray}\textit{0}} \\
{\color{gray}\textit{No source (lower bound)}} & {\color{gray}\textit{8.7 [6.0, 12.4]}} & {\color{gray}\textit{100.0}} & {\color{gray}\textit{42.0}} & {\color{gray}\textit{20.6}} & {\color{gray}\textit{0}} & {\color{gray}\textit{0}} & {\color{gray}\textit{not fitted}} & {\color{gray}\textit{0.071}} & {\color{gray}\textit{0}} \\
\bottomrule
\end{tabular}
\caption{Per-context details, GPT-5.6, 300 issues (file-level BM25 is in Table~\ref{tab:main}). Res.$|$app.: resolution among issues whose patch applied. In $\pm$2\%: share of issues whose context is within 2\% of $B_i$; ``not fitted'': contexts not cut to $B_i$. \$/issue: API cost of the whole pipeline for that context (localization draws, planner and patch call; list prices). Build s: median wall-clock seconds per issue to build the context with a model-based compressor or retriever (A6000 GPU, or CPU for LLMLingua-2). Bounds in grey italic.}
\label{tab:arms}
\end{table*}


==> generated/table_claude.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lrrrrr}
\toprule
Context & GPT & Claude & Applies & Res.$|$app. & Tokens \\
\midrule
Ours (CQ2-CARE) & 43.7 & 46.7 & 83.3 & 56.0 & 27.1K \\
Single draw (Q50-CARE) & 46.3 & 43.0 & 78.7 & 54.7 & 37.0K \\
Single draw, size-matched & 42.7 & 48.3 & 83.7 & 57.8 & 28.1K \\
LLMLingua-2 & 30.0 & 40.3 & 80.7 & 50.0 & 26.5K \\
LongLLMLingua & 35.0 & 29.0 & 63.0 & 46.0 & 26.7K \\
LongCodeZip & 37.3 & 36.0 & 73.3 & 49.1 & 26.2K \\
BM25 (chunks) & 29.0 & 34.0 & 82.3 & 41.3 & 26.9K \\
Dense (chunks) & 22.7 & 33.7 & 86.7 & 38.8 & 27.0K \\
BM25 (files) & 34.3 & 34.0 & 80.7 & n/a & 26.3K \\
{\color{gray}\textit{Gold files (upper bound)}} & {\color{gray}\textit{49.3}} & {\color{gray}\textit{46.3}} & {\color{gray}\textit{83.0}} & {\color{gray}\textit{55.8}} & {\color{gray}\textit{12.2K}} \\
{\color{gray}\textit{No source (lower bound)}} & {\color{gray}\textit{8.7}} & {\color{gray}\textit{13.0}} & {\color{gray}\textit{81.0}} & {\color{gray}\textit{16.0}} & {\color{gray}\textit{0.0K}} \\
\bottomrule
\end{tabular}
\caption{The 300 issues with GPT-5.6 and with Claude Opus 5 for every call (resolved \%). Applies, Res.$|$app. and Tokens are for Claude. Bounds in grey italic.}
\label{tab:claude}
\end{table*}


==> generated/table_controlled.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2.4pt}
\begin{tabular}{lrrrr@{}l}
\toprule
Context & $\varepsilon$ & App. & Res. & \multicolumn{2}{c}{$\Delta$} \\
\midrule
\multicolumn{6}{l}{\textbf{(a) All 300 issues}} \\
\textbf{Ours (CQ2-CARE)} & 100.0 & 98.0 & 43.7 &  &  \\
\quad second patch sample & 100.0 & 98.0 & 43.7 & 0.0 &  \\
\quad all lines corrupted & 0.3 & 78.7 & 34.0 & $-$9.7 & $^{***}$ \\
\multicolumn{6}{l}{\emph{From a single draw (main study):}} \\
\quad LongCodeZip & 96.8 & 89.7 & 37.3 & $-$6.3 & $^{**}$ \\
\quad LLMLingua-2, tokens & 17.5 & 70.7 & 30.0 & $-$13.7 & $^{***}$ \\
\multicolumn{6}{l}{\emph{Control: our candidate files, then compressed:}} \\
\quad LongCodeZip & 98.3 & 95.7 & 44.7 & +1.0 &  \\
\quad LLMLingua-2, lines & 100.0 & 89.7 & 40.7 & $-$3.0 &  \\
\quad LLMLingua-2, tokens & 41.2 & 80.0 & 36.3 & $-$7.3 & $^{**}$ \\
\midrule
\multicolumn{6}{l}{\textbf{(b) 100-issue subset}} \\
\textbf{Ours (CQ2-CARE)} & 100.0 & 98.0 & 41.0 &  &  \\
\quad second patch sample & 100.0 & 98.0 & 44.0 & +3.0 &  \\
\quad 25\% lines corrupted & 76.1 & 85.0 & 39.0 & $-$2.0 &  \\
\quad 50\% lines corrupted & 51.5 & 83.0 & 35.0 & $-$6.0 &  \\
\quad all lines corrupted & 0.4 & 80.0 & 38.0 & $-$3.0 &  \\
LLMLingua-2, tokens & 23.2 & 71.0 & 28.0 &  &  \\
\quad whole lines & 100.0 & 86.0 & 36.0 & +8.0 & $^{**}$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Controlled tests of verbatim text and gold-file recall} (GPT-5.6, post hoc). Corrupted rows: our own files with a share of lines each losing 20\% of their tokens. Control rows (our candidate files, then compressed) are not competing baselines: the compressors cut the union of our two localization draws with our evidence step to $B_i$, so they inherit our file choice and only the cut differs. Whole lines: LLMLingua-2's own token scores averaged per line, whole verbatim lines kept up to $B_i$. $\Delta$: resolution minus that of the nearest unindented row above (points); $\varepsilon$ (verbatim lines), App.\ (patches apply) and Res.\ (resolved) in \%; $^{***}p<0.001$, $^{**}p<0.01$, $^{*}p<0.05$ in two-sided exact McNemar tests.}
\label{tab:controlled}
\end{table}


==> generated/table_loc.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lrrrr}
\toprule
Localized set & Files & Precision & Recall & F1 \\
\midrule
Single draw (Q50) & 3.40 & 0.367 & 0.650 & 0.430 \\
Single draw, size-matched & 1.69 & 0.696 & 0.608 & 0.600 \\
Two-draw agreement (ours) & 1.71 & 0.705 & 0.631 & 0.613 \\
Union of two draws & 2.23 & 0.655 & 0.674 & 0.596 \\
1-of-5 agreement & 2.53 & 0.627 & 0.689 & 0.584 \\
2-of-5 agreement & 2.15 & 0.673 & 0.680 & 0.610 \\
3-of-5 agreement & 1.89 & 0.698 & 0.658 & 0.617 \\
4-of-5 agreement & 1.71 & 0.717 & 0.638 & 0.623 \\
5-of-5 agreement & 1.59 & 0.716 & 0.604 & 0.607 \\
\bottomrule
\end{tabular}
\caption{Changed-file localization against the pre-existing files the gold patch modifies (mean 1.86 per issue), 300 issues, GPT-5.6. Two-draw agreement beats a single draw by +0.184 F1 [+0.161, +0.206], but a single draw cut to the same size is within 0.013 [-0.005, +0.031].}
\label{tab:loc}
\end{table}


==> generated/table_main.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrrr@{\extracolsep{0pt}}l@{\extracolsep{\fill}\hspace{10pt}}rrrrrr@{\extracolsep{0pt}}l@{\extracolsep{\fill}}}
\toprule
 & \multicolumn{7}{c}{GPT-5.6} & \multicolumn{7}{c}{Claude Opus 5} \\
\cmidrule(lr){2-8}\cmidrule(lr){9-15}
Context & Tok. & $\varepsilon$ & $\rho$ & App. & Res.$\uparrow$ & \multicolumn{2}{c}{$\Delta$} & Tok. & $\varepsilon$ & $\rho$ & App. & Res.$\uparrow$ & \multicolumn{2}{c}{$\Delta$} \\
\midrule
\textbf{Ours (CQ2-CARE)} & 13.8 & 100.0 & 79.0 & 98.0 & \textbf{43.7} &  &  & 27.1 & 100.0 & 84.0 & 83.3 & \textbf{46.7} &  &  \\
LLMLingua-2 & 13.1 & 17.5 & 78.3 & 70.7 & 30.0 & $-$13.7 & $^{***}$ & 26.5 & 8.2 & 84.3 & 80.7 & 40.3 & $-$6.3 & $^{*}$ \\
LongLLMLingua & 13.2 & 67.1 & 63.7 & 84.0 & 35.0 & $-$8.7 & $^{***}$ & 26.7 & 69.9 & 73.1 & 63.0 & 29.0 & $-$17.7 & $^{***}$ \\
LongCodeZip & 13.1 & 96.8 & 72.2 & 89.7 & 37.3 & $-$6.3 & $^{**}$ & 26.2 & 96.9 & 82.9 & 73.3 & 36.0 & $-$10.7 & $^{***}$ \\
BM25 (chunks) & 13.6 & 100.0 & 58.3 & 86.7 & 29.0 & $-$14.7 & $^{***}$ & 26.9 & 100.0 & 71.9 & 82.3 & 34.0 & $-$12.7 & $^{***}$ \\
Dense (chunks) & 13.7 & 100.0 & 57.9 & 78.3 & 22.7 & $-$21.0 & $^{***}$ & 27.0 & 100.0 & 68.4 & 86.7 & 33.7 & $-$13.0 & $^{***}$ \\
BM25 (files) & 12.9 & 100.0 & 49.8 & 95.7 & 34.3 & $-$9.3 & $^{***}$ & 26.3 & 100.0 & 58.2 & 80.7 & 34.0 & $-$12.7 & $^{***}$ \\
\midrule
{\color{gray}\textit{Gold files (upper)}} & {\color{gray}\textit{12.2}} & {\color{gray}\textit{100.0}} & {\color{gray}\textit{97.0}} & {\color{gray}\textit{97.7}} & {\color{gray}\textit{49.3}} &  &  & {\color{gray}\textit{12.2}} & {\color{gray}\textit{100.0}} & {\color{gray}\textit{97.0}} & {\color{gray}\textit{83.0}} & {\color{gray}\textit{46.3}} &  &  \\
{\color{gray}\textit{No source (lower)}} & {\color{gray}\textit{0}} & {\color{gray}\textit{n/a}} & {\color{gray}\textit{0.0}} & {\color{gray}\textit{42.0}} & {\color{gray}\textit{8.7}} &  &  & {\color{gray}\textit{0}} & {\color{gray}\textit{n/a}} & {\color{gray}\textit{0.0}} & {\color{gray}\textit{81.0}} & {\color{gray}\textit{13.0}} &  &  \\
\bottomrule
\end{tabular*}
\caption{\textbf{At the same per-issue token budget, exact whole files beat token compressors and retrieval.} Every compressed or retrieved context is fitted to the realized size $B_i$ of our context for that model on each issue (\S\ref{sec:setup}); file-level BM25 adds whole files while they fit, so it lands under $B_i$. Tok.: mean context tokens (thousands); $\varepsilon$: verbatim lines; $\rho$: gold-file recall; App.: patches that apply; Res.: resolved, official tests pass; all in \% except Tok. Bold: best resolution per model; the gold files (upper bound) and the no-source context (lower bound), in grey italic, are references, not competing methods, and get no $\Delta$; the no-source context has no lines. $\Delta$: the row's resolution minus ours (points), so ours has none; $^{***}p<0.001$, $^{**}p<0.01$, $^{*}p<0.05$ in one-sided exact McNemar tests (alternative: ours resolves more), Holm-adjusted within the compressors and within the planned retrievers. File-level BM25 was added after the main results; its tests are unadjusted.}
\label{tab:main}
\end{table*}


==> generated/table_robust.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lr@{\extracolsep{0pt}}l@{\extracolsep{\fill}}r@{\extracolsep{0pt}}l}
\toprule
 & \multicolumn{4}{c}{Gap to ours (points)} \\
\cmidrule(l){2-5}
Baseline & \multicolumn{2}{c}{In tolerance} & \multicolumn{2}{c}{Search/replace} \\
\midrule
LLMLingua-2 & $-$16.7 & $^{***}$ & $-$15.0 & $^{***}$ \\
LongLLMLingua & $-$11.6 & $^{***}$ & $-$13.0 & $^{**}$ \\
LongCodeZip & $-$6.6 & $^{**}$ & $-$9.0 & $^{*}$ \\
BM25 (chunks) & $-$14.6 & $^{***}$ & $-$19.0 & $^{***}$ \\
Dense (chunks) & $-$20.9 & $^{***}$ & $-$17.0 & $^{***}$ \\
\bottomrule
\end{tabular*}
\caption{\textbf{The baselines still trail ours in two further checks} (GPT-5.6). Gap to ours: the baseline's resolution minus ours. In tolerance: only the issues where the baseline's realized tokens are within $\pm$2\% of $B_i$ (197--297 of 300 per baseline; Holm-adjusted). Search/replace: both contexts with exact-match search/replace edits instead of diffs (100 issues, unadjusted). $^{***}p<0.001$, $^{**}p<0.01$, $^{*}p<0.05$ in one-sided exact McNemar tests (alternative: ours resolves more).}
\label{tab:robust}
\end{table}


==> generated/table_variants.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2.4pt}
\begin{tabular}{@{}lrrrrr@{}l@{}}
\toprule
Context & Files & F1 & Tok. & Res. & \multicolumn{2}{c}{$\Delta$} \\
\midrule
\textbf{Ours}: both draws name & 1.71 & 0.613 & 13.8 & 43.7 &  &  \\
\multicolumn{7}{@{}l}{\emph{Fewer files without agreement:}} \\
\quad One draw, same file count & 1.69 & 0.600 & 13.3 & 42.7 & $-$1.0 &  \\
\multicolumn{7}{@{}l}{\emph{More files:}} \\
\quad One draw, all files & 3.40 & 0.430 & 20.1 & 46.3 & +2.7 &  \\
\quad Either draw names & 2.23 & 0.596 & 16.1 & 47.7 & +4.0 & $^{*}$ \\
\multicolumn{7}{@{}l}{\emph{No evidence spans:}} \\
\quad Ours without evidence & 1.71 & 0.613 & 10.4 & 40.7 & $-$3.0 &  \\
\bottomrule
\end{tabular}
\caption{\textbf{Agreement helps only by selecting fewer files} (GPT-5.6, 300 issues). The rows change how the files are chosen, or drop the evidence spans. Ours keeps the files that both of two localization draws name; one draw cut to the same number of files does about as well, while showing more files resolves more at more tokens, and dropping the evidence spans costs 3.0 points. Files: selected files per issue; F1: changed-file F1 against the files the gold patch modifies; Tok.: mean context tokens (thousands); Res.: resolved (\%); $\Delta$: row minus ours (points); $^{*}p<0.05$ in two-sided exact McNemar tests.}
\label{tab:variants}
\end{table}


==> generated/table_w2.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrrrrrrr}
\toprule
\multicolumn{8}{l}{\emph{(a) By issue creation date (terciles of 100)}} \\
Created & No source & Ours & \multicolumn{5}{c}{row minus ours} \\
 & & & LLMLingua-2 & LongLLMLingua & LongCodeZip & BM25 (chunks) & Dense (chunks) \\
\midrule
2025-01--2025-04 & 10.0 & 48.0 & $-$14.0 & $-$6.0 & $-$6.0 & $-$12.0 & $-$24.0 \\
2025-04--2025-10 & 8.0 & 41.0 & $-$14.0 & $-$6.0 & $-$3.0 & $-$17.0 & $-$15.0 \\
2025-10--2026-05 & 8.0 & 42.0 & $-$13.0 & $-$14.0 & $-$10.0 & $-$15.0 & $-$24.0 \\
\midrule newest $-$ oldest & & & +1.0 & $-$8.0 & $-$4.0 & $-$3.0 & 0.0 \\
\quad 95\% CI & & & $-$11.0, +12.0 & $-$18.0, +2.0 & $-$15.0, +7.0 & $-$15.0, +9.0 & $-$12.0, +13.0 \\
\midrule
\multicolumn{8}{l}{\emph{(b) Within-issue regression of resolution (coefficient [95\% CI])}} \\
 & \multicolumn{3}{r}{without applies} & \multicolumn{4}{r}{with applies} \\
\midrule
Verbatim lines $\varepsilon$ & \multicolumn{3}{r}{+0.146 [+0.103, +0.190]} & \multicolumn{4}{r}{+0.043 [+0.002, +0.080]} \\
Gold-file recall $\rho$ & \multicolumn{3}{r}{+0.273 [+0.213, +0.333]} & \multicolumn{4}{r}{+0.213 [+0.158, +0.272]} \\
log tokens & \multicolumn{3}{r}{$-$0.030 [$-$0.054, $-$0.008]} & \multicolumn{4}{r}{$-$0.031 [$-$0.053, $-$0.009]} \\
Patch applies & \multicolumn{3}{r}{not in model} & \multicolumn{4}{r}{+0.342 [+0.276, +0.411]} \\
\bottomrule
\end{tabular}
\caption{\textbf{Post-hoc offline checks} (GPT-5.6, 300 issues). (a) Resolution (\%) of the no-source context and of ours by issue creation date, and each baseline's resolution minus ours (points); a gap driven by memorized fixes would shrink on newer issues. (b) Linear probability model of resolution with issue fixed effects over all 3,298 (issue, context) pairs that show source; the right column adds whether the patch applies. Intervals: 2,000-draw issue bootstrap.}
\label{tab:w2}
\end{table*}

